An Analysis of Logit Learning with the r-Lambert Function

The well-known replicator equation in evolutionary game theory describes how population-level behaviors change over time when individuals make decisions using simple imitation learning rules. In this paper, we study evolutionary dynamics based on a fundamentally different class of learning rules known as logit learning. Numerous previous studies on logit dynamics provide numerical evidence of bifurcations of multiple fixed points for several types of games. Our results here provide a more explicit analysis of the logit fixed points and their stability properties for the entire class of two-strategy population games -- by way of the $r$-Lambert function. We find that for Prisoner's Dilemma and anti-coordination games, there is only a single fixed point for all rationality levels. However, coordination games exhibit a pitchfork bifurcation: there is a single fixed point in a low-rationality regime, and three fixed points in a high-rationality regime. We provide an implicit characterization for the level of rationality where this bifurcation occurs. In all cases, the set of logit fixed points converges to the full set of Nash equilibria in the high rationality limit.

==> Lemmas/Lma-h0h1rts.tex <==
If $\delta_{RT0} > -\delta_{SP0}$ and $(\delta_{SP0},\delta_{RT0}) \in \mathcal{Q}_{\text{\rom{2}}}$, $h_{-1}(\beta) < 0$ for all $\beta > -\frac{2}{\delta_{SP}}$, and there exists one root $\beta_{r,0} > -\frac{2}{\delta_{SP}}$ for $h_0(\beta)$.  This root is given implicitly by \[
W_0(-e^{\beta_{r,0} \delta_{SP} + 1}) = 1 - \frac{\beta_{r,0} m}{2} + \frac{\sqrt{\beta_{r,0} m\left(\beta_{r,0} m - 4\right)}}{2}.
\]

Furthermore, if $\delta_{RT0} > -\delta_{SP0}$ and $(\delta_{SP0},\delta_{RT0}) \in \mathcal{Q}_{\text{\rom{2}}}$, the function $h_0(\beta)\geq0$ for all $\beta \geq \beta_{r,0} > -\frac{2}{\delta_{SP}}$ such that \[
W_0(-re) \geq 1 - \frac{\beta m}{2} + \frac{\sqrt{\beta m\left(\beta m - 4\right)}}{2},
\]
and $h_0(\beta)<0$ for all $-\frac{2}{\delta_{SP}} \leq \beta < \beta_{r,0}$ such that \[
W_0(-re) < 1 - \frac{\beta m}{2} + \frac{\sqrt{\beta m\left(\beta m - 4\right)}}{2} .
\]

If $0 < \delta_{RT} < -\delta_{SP}$ and $(\delta_{SP},\delta_{RT}) \in \mathcal{Q}_{\text{\rom{2}}}$, $h_{0}(\beta) > 0$ for all $\beta > -\frac{2}{\delta_{SP}}$, and there exists one root $\beta_{r,-1} > -\frac{2}{\delta_{SP}}$ for $h_{-1}(\beta)$.  This root is given implicitly by \[
W_{-1}(-e^{\beta_{r,-1} \delta_{SP} + 1}) = 1 - \frac{\beta_{r,-1} m}{2} - \frac{\sqrt{\beta_{r,-1} m\left(\beta_{r,-1} m - 4\right)}}{2}.
\]

Furthermore, if $0 < \delta_{RT0} < -\delta_{SP0}$ and $(\delta_{SP0},\delta_{RT0}) \in \mathcal{Q}_{\text{\rom{2}}}$, the function $h_{-1}(\beta)\leq0$ for all $\beta > \beta_{r,-1} > -\frac{2}{\delta_{SP}}$ such that \[
W_{-1}(-re) \geq 1 - \frac{\beta m}{2} - \frac{\sqrt{\beta m\left(\beta m - 4\right)}}{2},
\]
and $h_{-1}(\beta)>0$ for all $-\frac{2}{\delta_{SP}} < \beta < \beta_{r,-1}$ such that \[
W_{-1}(-re) < 1 - \frac{\beta m}{2} - \frac{\sqrt{\beta m\left(\beta m - 4\right)}}{2}.
\]

If $\delta_{RT0} = -\delta_{SP0}$, then there exist no roots $\beta_r \in \mathbb{D}_2$ .  The function $h_0(\beta)>0$ and the function $h_{-1}(\beta)<0$ for all $\beta > -\frac{2}{\delta_{SP}}$.

==> Proofs/No_Of_Fixed_Points/prf-NoOfFps_short.tex <==
By \cite[Theorem 4]{mezHo2017generalization}, the number of solutions to the $r$-Lambert function depends on the value of $r$.
\begin{itemize}
\item There is one solution if $r \geq e^{-2}$
\item There are at most three solutions if $0 < r < e^{-2}$
\item There are two solutions if $r < 0$.
\end{itemize}

As $r = e^{\beta \delta_{SP}}$, one knows that $r$ is never less than or equal to zero for all $\beta \geq 0$ and any $\delta_{SP}\in\mathbb{R}$.  Solving for when $r \geq e^{-2}$,
\begin{equation*}
r \geq e^{-2} \implies \begin{cases} \beta \geq -\frac{2}{\delta_{SP}} & \delta_{SP}>0 \\
\beta \leq -\frac{2}{\delta_{SP}} & \delta_{SP}<0
\end{cases}
\end{equation*}

If $\delta_{SP}>0$ then $-\frac{2}{\delta_{SP}}<0$.  As $\beta$ must be greater than zero by the definition of this system, for any model with $\delta_{SP}>0$, there will be only one solution.  Hence, there is only one solution when $(\delta_{SP},\delta_{RT})\in\mathcal{Q}_{\text{\rom{1}}}\cup\mathcal{Q}_{\text{\rom{4}}}$.

On the other hand, for models with $(\delta_{SP},\delta_{RT})\in\mathcal{Q}_{\text{\rom{2}}}\cup\mathcal{Q}_{\text{\rom{3}}}$, $\delta_{SP}<0$ and $-\frac{2}{\delta_{SP}}>0$.  Therefore, there is an interval $[0,-\frac{2}{\delta_{SP}}]$ wherein there is guaranteed to be only one solution, but for all $\beta > -\frac{2}{\delta_{SP}}$, there are at most three solutions.

Define $\alpha_r := W_{-1}(-re) - 1$, $\beta_r := W_{0}(-re) - 1$, and $f_r(z) = ze^z + rz$ as in \cite[Theorem 4]{mezHo2017generalization}.  By \cite[Theorem 4]{mezHo2017generalization},
\begin{itemize}
\item If $kr > f_r(\alpha_r)\$ or $kr < f_r(\beta_r)$, then there is one solution;
\item If $kr = f_r(\alpha_r)$ or $kr = f_r(\beta_r)$, then there there are two solutions; and 
\item $f_r(\beta_r) < kr < f_r(\alpha_r)$, then there are three solutions.
\end{itemize}

For $\delta_{RT}-\delta_{SP} \leq 0$, $kr=-\beta(\delta_{RT}-\delta_{SP})e^{\beta \delta_{SP}} > 0$ all $\beta \geq 0$.  By \cite{mezHo2017generalization}, the function $f_r(z)$ has one zero at $f_r(0)$ and is strictly increasing over the interval $[\beta_r,\infty)$.  Note the $f_r(\beta_r),f_r(\alpha_r) < 0$.  As $f_r(\beta_r)<f_r(\alpha_r)<0$ and as $kr > 0$ for all $\beta \geq0$, it follows that $kr > f_r(\alpha_r)$ for all $\beta \geq 0$.  Therefore, there is only one solution for $(\delta_{SP},\delta_{RT})\in\mathcal{Q}_{\text{\rom{3}}}\setminus\left\{ (\delta_{SP},\delta_{RT}) \; \middle| \; \delta_{RT} > \delta_{SP} \right\}$.

For $(\delta_{SP},\delta_{RT})\in\mathcal{Q}_{\text{\rom{2}}}\cup\mathcal{Q}_{\text{\rom{3}}}\setminus\left\{ (\delta_{SP},\delta_{RT}) \; \middle| \; \delta_{RT} \leq \delta_{SP} \right\}$, however, $kr<0$ for all $\beta >0$.  In this case, there is one solution if $kr > f_r(\alpha_r)$ or $kr < f_r(\beta_r)$.  These expressions simplify to
\begin{align*}
h_{-1}(\beta) &> 0 \\
h_{0}(\beta) &< 0
\end{align*}
where $h_i(\beta):=W_i^2(-re) + (\beta m - 2)W_i(-re) + 1$ for $i=0,-1$.

\begin{lemma}[Stationary Points of $h_i(\beta)$]\label{lma:h0h1sps}
\input{./Lemmas/Lma-h0h1sps}
\end{lemma}

\begin{proof}
See Appendix *****
\end{proof}


For all $(\delta_{SP},\delta_{RT}) \in \mathcal{Q}_{\text{\rom{3}}}$ there are no stationary points.  Taking the limits as $\beta$ tends towards the extremes of the interval $(-\frac{2}{\delta_{SP}},\infty)$ over which there can be multiple solutions, one finds 
\begin{equation*}
\lim_{\beta\to -\frac{2}{\delta_{SP}}} h_i(\beta) = 2\left( \frac{\delta_{RT} + \delta_{SP}}{\delta_{SP}} \right) > 0, \ i=0,-1
\end{equation*}
and 
\begin{equation*}
\lim_{\beta\to \infty} h_0(\beta) = 1, \ \lim_{\beta\to \infty} h_{-1}(\beta) = \infty.
\end{equation*}
As both $h_0(\beta)$ and $h_{-1}(\beta)$ no stationary points and are always positive-valued in this parameter regime, each function monotonically tends toward its respective limit values. As such, the inequalities $kr > f_r(\alpha_r)$ and $kr > f_r(\beta_r)$ are true for all $\beta \geq0$ and for all $(\delta_{SP},\delta_{RT}) \in \mathcal{Q}_{\text{\rom{3}}}$.  Therefore, there is only one fixed point for all $\beta \geq 0$ and for all $(\delta_{SP},\delta_{RT}) \in \mathcal{Q}_{\text{\rom{3}}}$.

Furthermore, for all $(\delta_{SP},\delta_{RT})$ in the set
\begin{equation*}
(\delta_{SP},\delta_{RT}) \in \mathcal{Q}_{\text{\rom{2}}}\setminus\left\{ (\delta_{SP},\delta_{RT}) \; \middle| \; \delta_{RT} \leq -\delta_{SP} \right\}
\end{equation*}
there are also no stationary points.  Furthermore, taking the limits as $\beta$ tends towards the extremes of the interval $(-\frac{2}{\delta_{SP}},\infty)$ over which there can be multiple solutions, one finds 
\begin{equation*}
\lim_{\beta\to -\frac{2}{\delta_{SP}}} h_i(\beta) = 2\left( \frac{\delta_{RT} + \delta_{SP}}{\delta_{SP}} \right) < 0, \ i=0,-1
\end{equation*}
and 
\begin{equation*}
\lim_{\beta\to \infty} h_0(\beta) = 1, \ \lim_{\beta\to \infty} h_{-1}(\beta) = -\infty.
\end{equation*}

As there are no stationary points, $h_0(\beta)$ and $h_{-1}(\beta)$ must tend monotonically to $1$ and $-\infty$, respectively, from $2\left( \frac{\delta_{RT} + \delta_{SP}}{\delta_{SP}} \right)$, which is less than zero.  As such, $h_{-1}(\beta)$ is always less than zero, and $h_0(\beta)$ has one root $\beta_{r}$, past which $h_0(\beta)>0$ and before which $h_0(\beta)<0$.  Therefore, there are three fixed points for all $\beta > \beta_r > -\frac{2}{\delta_{SP}}$, there are two fixed points for $\beta = \beta_r$, and there is one fixed point for all $0 \leq \beta \leq -\frac{2}{\delta_{SP}}$.

For all $(\delta_{SP},\delta_{RT})$ in the set
\begin{equation*}
(\delta_{SP},\delta_{RT}) \in \mathcal{Q}_{\text{\rom{2}}}\setminus\left\{ (\delta_{SP},\delta_{RT}) \; \middle| \; \delta_{RT} \neq -\delta_{SP} \right\}
\end{equation*}
there are also no stationary points.  The limits as $\beta$ tends towards the extremes of the interval $(-\frac{2}{\delta_{SP}},\infty)$ over which there can be multiple solutions are
\begin{equation*}
\lim_{\beta\to -\frac{2}{\delta_{SP}}} h_i(\beta) = 2\left( \frac{\delta_{RT} + \delta_{SP}}{\delta_{SP}} \right) = 0, \ i=0,-1
\end{equation*}
and 
\begin{equation*}
\lim_{\beta\to \infty} h_0(\beta) = 1, \ \lim_{\beta\to \infty} h_{-1}(\beta) = -\infty.
\end{equation*}
As there are no stationary points, both $h_0(\beta)$ and $h_{-1}(\beta)$ tend monotonically towards $1$ and $-\infty$, respectively, from $0$.  Therefore, over the interval $\beta \in (-\frac{2}{\delta_{SP}},\infty)$, there are no zeros, and there are three fixed points for all $\beta > -\frac{2}{\delta_{SP}}$ and one fixed point for all $0 \leq \beta \leq -\frac{2}{\delta_{SP}}$.

For all $(\delta_{SP},\delta_{RT})$ in the set
\begin{equation*}
(\delta_{SP},\delta_{RT}) \in \mathcal{Q}_{\text{\rom{2}}}\setminus\left\{ (\delta_{SP},\delta_{RT}) \; \middle| \; \delta_{RT} \geq -\delta_{SP} \right\}
\end{equation*}
both $h_0(\beta)$ and $h_{-1}(\beta)$ have one stationary point in for $\beta \in (-\frac{2}{\delta_{SP}},\infty)$.  The limits as $\beta$ tends towards the extremes of the interval $(-\frac{2}{\delta_{SP}},\infty)$ over which there can be multiple solutions are
\begin{equation*}
\lim_{\beta\to -\frac{2}{\delta_{SP}}} h_i(\beta) = 2\left( \frac{\delta_{RT} + \delta_{SP}}{\delta_{SP}} \right) > 0, \ i=0,-1
\end{equation*}
and 
\begin{equation*}
\lim_{\beta\to \infty} h_0(\beta) = 1, \ \lim_{\beta\to \infty} h_{-1}(\beta) = -\infty.
\end{equation*}

Clearly from these limits and due to the presence of stationary points for $h_0(\beta)$ and $h_{-1}(\beta)$ in this parameter regime, there are potentially roots to $h_i(\beta)$, $i=0,-1$.
\begin{lemma}[Roots of $h_i(\beta)$]\label{lma:h0h1rts}
\input{./Lemmas/Lma-h0h1rts}
\end{lemma}

==> Proofs/Stability_of_Fixed_Points/Prf-AsympFPStab.tex <==
A fixed point of \eqref{eq:logit_dyn} is stable if $\left.\frac{df}{dx} \right|_{x=\frac{1}{k}W_r(kr)} \leq 0$.  The expression for $\frac{df}{dx}$ is given by
\begin{equation*}
    \frac{df}{dx} = \frac{\beta m e^{- \beta \left(\delta_{SP} + m x\right)}}{\left(1 + e^{- \beta \left(\delta_{SP} + m x\right)}\right)^{2}} - 1.
\end{equation*}

The $x$ fixed points as $\beta$ tends to infinity are known.  Starting with $(\delta_{SP},\delta_{RT}) \in \mathcal{Q}_{\text{\rom{1}}}$,
\begin{equation*}
    \lim_{\beta \to \infty}\left. \frac{df}{dx} \right|_{x=1} = \lim_{\beta \to \infty} \left. \left(\frac{\beta m e^{- \beta \left(\delta_{SP} + m x\right)}}{\left(1 + e^{- \beta \left(\delta_{SP} + m x\right)}\right)^{2}} - 1 \right)\right|_{x=1}.
\end{equation*}
Evaluating this limit, one acquires
\begin{equation*}
    \lim_{\beta \to \infty}\left. \frac{df}{dx} \right|_{x=1} = -1 < 0.
\end{equation*}

Repeating this process for $(\delta_{SP},\delta_{RT}) \in \mathcal{Q}_{\text{\rom{4}}}$, the asymptotic fixed point is $x=-\frac{\delta_{SP}}{\delta_{RT}-\delta_{SP}}$.  By evaluating the limit $\lim_{\beta \to \infty} \frac{df}{dx}$ at this fixed point, one obtains
\begin{equation*}
     \lim_{\beta \to \infty}\left. \frac{df}{dx} \right|_{x=-\frac{\delta_{SP}}{\delta_{RT}-\delta_{SP}}} = -\infty < 0
\end{equation*}

Again, repeating this process for $(\delta_{SP},\delta_{RT}) \in \mathcal{Q}_{\text{\rom{3}}}$, the asymptotic fixed point is $x=0$.  By evaluating the limit $\lim_{\beta \to \infty} \frac{df}{dx}$ at this fixed point, one obtains
\begin{equation*}
     \lim_{\beta \to \infty}\left. \frac{df}{dx} \right|_{x=0} = -1 < 0
\end{equation*}

Finally, repeating this process for $(\delta_{SP},\delta_{RT}) \in \mathcal{Q}_{\text{\rom{2}}}$, the asymptotic fixed points are $x=0,1,-\frac{\delta_{SP}}{\delta_{RT}-\delta_{SP}}$.  By evaluating the limit $\lim_{\beta \to \infty} \frac{df}{dx}$ at the fixed points $x=0,1$, one obtains
\begin{equation*}
     \lim_{\beta \to \infty}\left. \frac{df}{dx} \right|_{x=0,1,} = -1 < 0
\end{equation*}

However, at the fixed point $-\frac{\delta_{SP}}{\delta_{RT}-\delta_{SP}}$, the limits evaluates $+\infty$ as $m>0$ for any point $(\delta_{SP},\delta_{RT})\in\mathcal{Q}_{\text{\rom{2}}}$.  Therefore, if $m>0$, then the fixed point $-\frac{\delta_{SP}}{\delta_{RT}-\delta_{SP}}$ is unstable.

Hence, all fixed points are stable unless the parameters reside in the region $(\delta_{SP},\delta_{RT}) \in \mathcal{Q}_{\text{\rom{2}}}\setminus\left\{ (\delta_{SP},\delta_{RT}) \; \middle| \; \delta_{RT} \leq \delta_{SP}\right\}$.  If the parameters reside in this region, however, $x=-\frac{\delta_{SP}}{\delta_{RT}-\delta_{SP}}$ is the only unstable fixed point.

==> Sec-NoOfFPs.tex <==


Analyzing the asymptotic tendencies of the fixed points, summarized in Theorem \ref{thm:AsympOfFPs}, yields the results of Theorem \ref{thm:NoOfFPs}.
\begin{theorem}[Fixed Point Values as $\beta \to \infty$]\label{thm:AsympOfFPs}
\input{./Theorems/thm-AsympOfFPs}
\end{theorem}
\begin{proof}
See Appendix \ref{ap:asympFP}
\end{proof}

Furthermore, and confirming Theorem \ref{thm:AsympOfFPs}, using the properties of the $r$-Lambert and Lambert W functions, one can deduce the number of fixed points per parameter regime as summarized in Theorem \ref{thm:NoOfFPs}. 
\begin{theorem}[The Number of Fixed Points]\label{thm:NoOfFPs}
\input{./Theorems/thm-NoOfFps}
\end{theorem}

\begin{proof}
\input{./Proofs/"No Of Fixed Points"/prf-NoOfFps_short2}
\end{proof}





%\begin{theorem}
%The values of the $x$ fixed points %converge monotonically to the values in %the set $\mathcal{S}_{fp,\infty}$.
%\end{theorem}

%\begin{proof}
%    I see this numerically and want to %prove it, but I haven't done so yet.
%\end{proof}

==> introduction.tex <==
% !TEX root = main.tex

Evolutionary game theory provides a wide range of tools to analyze how large populations of agents behave over time. Originating in the fields evolutionary biology and population dynamics \cite{taylor1978evolutionary,smith1982evolution}, these mathematical tools are now widely applicable to the study of societal and engineered systems too like traffic networks, distributed control systems, and social behaviors in epidemics \cite{smith1993new,quijano2017role,weitz2016oscillating,frieswijk2022modeling,gong2022limit,leonardos2023catastrophe,satapathi2023coupled}.  Central to an evolutionary game is the \emph{learning rule}, also called a \emph{revision protocol} \cite{sandholm2010population}, whereby individual agents choose their strategies during the game. When all agents adopt a particular learning rule, one can derive the associated mean dynamical equations that describe how the proportion of agents using a particular strategy changes over time.

Considering that evolutionary game theoretic tools are increasingly applied to model human population dynamics and large-scale socio-technical systems, it becomes increasingly important to study the impact of different learning rules on the game's population-level behavior. Perhaps the most well-studied and utilized protocol is the imitative revision protocol utilized in the replicator equation. Originally formulated to model biological replication and fitness \cite{taylor1978evolutionary}, the replicator equation is the mean dynamic of agents utilizing imitative learning rules.  In other words, the replicator equation models agents who only switch their strategy if they observe a more successful agent using a different strategy.

Therefore, imitators decide based on the perceived success or failure of those in their immediate vicinity.  They, by definition, do not assess the potential benefits of using the various means at their disposal. Intelligent decision-making does require this assessment, however.  Intelligent decision-making depends on the acquisition of information and rationally choosing a course of action based on the facts.

Information is readily available in abundance, and the amount thereof grows daily.  Clear examples that pervade society are the utilization of traffic information systems (Google Maps, Waze, etc), recommendation and search algorithms, and the consultation of AI-powered large language models.  As the amount information available to decision-makers increases, evolutionary game theoretic models reliant upon imitative learning rules will be able to accurately model fewer and fewer real-world system.  This, therefore, necessitates a revision protocol that models informed decision-making .

A learning rule that models informed decision-making is the \emph{logit learning} revision protocol.  Agents using this protocol know the payoffs of each strategy and weigh the payoffs of choosing one strategy against the payoffs of all the strategies. In other words, each agent decides what to do next using information on the advantages and disadvantages of any given course of action.  The logit learning rule represents the level at which the agents rationally make this choice using the information at hand using a rationality parameter $\beta \geq 0$.  When $\beta = 0$, agents choose their strategies uniformly at random, and increasing values of $\beta$ correspond to agents selecting payoff-maximizing strategies with higher probability.


The focus of this paper is on the analysis of logit learning dynamics in two-strategy population games. Our analysis centers on completely characterizing all fixed points and their stability properties for all possible two-strategy games. This includes dominant-strategy, anti-coordination, and coordination games. While such properties are well-known for the replicator dynamic, they are not systematically characterized for logit dynamics. This is primarily because the logit fixed points cannot be derived in a closed form. Consequently, many previous studies of logit dynamics primarily illustrate many interesting properties (e.g. bifurcations and limit cycles) via numerical simulations for specific games \cite{tuyls2003selection,hommes2012multiple,bloembergen2015evolutionary}. One recent work analyzes logit dynamics in general population games with control-theoretic tools \cite{cianfanelli2023logit}.

Our main contribution establishes a connection between two-strategy population games with logit dynamics and the Lambert W function. By leveraging properties of the Lambert W function, we are able to more precisely understand the behavior of logit fixed points as the rationality parameter $\beta$ is varied.

Preliminary background on evolutionary games is provided in Section \ref{sec:prelim}. 





==> preliminaries.tex <==
% !TEX root = main.tex


